Recognizing People by Body Shape Using Deep Networks of Images and Words

Common and important applications of person identification occur at distances and viewpoints in which the face is not visible or is not sufficiently resolved to be useful. We examine body shape as a biometric across distance and viewpoint variation. We propose an approach that combines standard object classification networks with representations based on linguistic (word-based) descriptions of bodies. Algorithms with and without linguistic training were compared on their ability to identify people from body shape in images captured across a large range of distances/views (close-range, 100m, 200m, 270m, 300m, 370m, 400m, 490m, 500m, 600m, and at elevated pitch in images taken by an unmanned aerial vehicle [UAV]). Accuracy, as measured by identity-match ranking and false accept errors in an open-set test, was surprisingly good. For identity-ranking, linguistic models were more accurate for close-range images, whereas non-linguistic models fared better at intermediary distances. Fusion of the linguistic and non-linguistic embeddings improved performance at all, but the farthest distance. Although the non-linguistic model yielded fewer false accepts at all distances, fusion of the linguistic and non-linguistic models decreased false accepts for all, but the UAV images. We conclude that linguistic and non-linguistic representations of body shape can offer complementary identity information for bodies that can improve identification in applications of interest.

==> Body_IJCB/scrape_to_paste.tex <==

% The following table identifies the models that we explore for comparison:
% \begin{center}
% \begin{tabular}{|l|l|}
% \hline
% Resnet-ImageNet & ResNet-LinguisticCore\\
% \hline\hline
% BRS1 & BRS1 \\
% BRS1, 1.1, 2 & BRS1, 1.1, 2\\
% BRS1, 1.1, 2, 3 & BRS1,1.1, 2, 3\\
% BRS1, 1.1, 2 + triplet loss & BRS1, 2 + triplet loss\\
% BRS1, 1.1, 2, 3 + triplet loss & BRS1, 1.1, 2, 3 + triplet loss\\
% \hline
% \end{tabular}
% \end{center}


% The first extended linguistic model (LingBRS1) is fine-tuned with 158 identities from BRS1 (46,834 images); the second (LingBRS12) is fine-tuned with  158 identities from BRS1, 54 identities from BRS1.1, and 195 identities from BRS2 (111,256 images); the third (LingBRS123) is fine-tuned with 158 identities from BRS1, 54 identities from BRS1.1, 195 identities from BRS2, and 170 identities from BRS3 (199,829 images).

% Likewise, extended object models (base pretrained ResNet 101 on ImageNet 1k) are fine tuned using the same datasets to generate comparisons. Thus for each extended linguistic model above there is a corresponding extended object model trained on the same data for comparison(ex. LingBRS1 and ObjBRS1 are both trained on BRS1 images). 



% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

%\ijcbfinalcopy 
% *** Uncomment this line for the final submission

\def\ijcbPaperID{****} % *** Enter the IJCB Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
%\ifijcbfinal\pagestyle{empty}\fi

% Thus, for example, 
% in a recent study \cite{geirhos2018imagenet}, a DCNN trained on ImageNet \cite{imagenet} classified a picture of a cat, with fur replaced by elephant skin, as an elephant. This texture bias makes the learning of global body shape (independent of clothing color and texture) especially challenging.  

%-------------------------------------------------------------------------

% Consider $V_{i,j} = \{ f_{1_{ij}}, f_{2_{ij}}, f_{3_{ij}}, ..., f_{n_{ij}} \}$ as the set of frames composing a video $V_i$ of a given identity $j$. Supposing that $\tau_\theta$ is the perfect classifier, we would expect that $\tau_{\theta}(f_{k_{ij}}) = \tau_{\theta}(f_{k_{ij}}) \: \forall$ image pairs $\ni k \ne k$, $i \ne i$, but $j = j$ (same identity pairs). Subject to image variance, and the task specific need to classify never seen before bodies, we defer to distance metrics in place of equality and expect that for a very good classifier, $\tau_{\hat{\theta}}$, the distance between $({\tau_\theta(f_{k_{ij}})}, {\tau_\theta(f_{k_{ij}})}) \: \forall$ image pairs $\ni k \ne k$, $i \ne i$, but $j = j$ will be small. With high dimensional output layers ($>$512), we opt to use cosine similarity between network outputs as the metric for how similarly a network encodes two identities. 

%Consider \begin{math} Vi,j = \{f_{1\i\j},f_{2\i\j},f_{3\i\j},...,f_{n\i\j} \end{math} as the set of frames composing a video Vi of a given identity j. Supposing that \begin{math} {\tau_\theta} \end{math} is the perfect classifier, we would expect that \begin{math} {\tau_\theta(f_{k\i\j}) = \tau_\theta(f_{k\i\j}) \forall image-pairs \ni k \ne k, i \ne i, but j = j} \end{math} (same identity pairs). Subject to image variance, and the task specific need to classify never seen before bodies, we defer to distance metrics in place of equality and expect that for a very good classifier, \begin{math}\tau__{\hat{\theta}}\end{math}, the distance between \begin{math}({\tau_\theta(f_{k\i\j})},{\tau_\theta(f_{k\i\j})}) \forall image-pairs \ni k \ne k, i \ne i, but j = j\end{math} will be small. With high dimensional output layers(>512), we opt to use cosine similarity between network outputs as the metric for how similarly a network encodes two identities. 


% \begin{table*}
% \begin{center}
% \begin{tabular}{|l|c|c|}
% \hline
% Subset & ID Count & Distances \\
% \hline\hline
% BRS1 & 158 & 100m, 200m, 400m, 500m, and UAV \\
% BRS1.1 & 54 & 100m, 300m, 400m, 500m, and UAV \\
% BRS2 & 195 & 100m, 270m, 370m, 800m, and 1000m\\
% BRS3 & 170 & 100m, 200m, 300m, and 500m\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Subsets of the BRS dataset}
% \end{table*}




\begin{comment}
BRS1, BRS1.1, BRS2, and BRS3. BRS1 contains 158 identities. The field set for BRS1 consists of videos recorded at various ranges: close range, 100 meters, 200 meters, 400 meters, 500 meters, and unmanned aerial vehicle (UAV).

BRS1.1 contains 54 identities and consists of videos recorded at close range, 100 meters, 300 meters, 400 meters, 500 meters, and UAV.

BRS2 contains 195 identities and consists of videos recorded at close range, 100 meters, 270 meters, 370 meters, 800 meters, and 1000 meters.

BRS3 contains 170 identities and consists of videos recorded at close range, 100 meters, 200 meters, 300 meters, 400 meters, and 500 meters.
\end{comment}


